Recurrent and Spiking Modeling of Sparse Surgical Kinematics

Robot-assisted minimally invasive surgery is improving surgeon performance and patient outcomes. This innovation is also turning what has been a subjective practice into motion sequences that can be precisely measured. A growing number of studies have used machine learning to analyze video and kinematic data captured from surgical robots. In these studies, models are typically trained on benchmark datasets for representative surgical tasks to assess surgeon skill levels. While they have shown that novices and experts can be accurately classified, it is not clear whether machine learning can separate highly proficient surgeons from one another, especially without video data. In this study, we explore the possibility of using only kinematic data to predict surgeons of similar skill levels. We focus on a new dataset created from surgical exercises on a simulation device for skill training. A simple, efficient encoding scheme was devised to encode kinematic sequences so that they were amenable to edge learning. We report that it is possible to identify surgical fellows receiving near perfect scores in the simulation exercises based on their motion characteristics alone. Further, our model could be converted to a spiking neural network to train and infer on the Nengo simulation framework with no loss in accuracy. Overall, this study suggests that building neuromorphic models from sparse motion features may be a potentially useful strategy for identifying surgeons and gestures with chips deployed on robotic systems to offer adaptive assistance during surgery and training with additional latency and privacy benefits.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> backup_text.tex <==
\label{mimic-data}
\begin{figure}[!tbph]
  \centering
\includegraphics[width=\textwidth]{imgs/PickPlace.png}
\caption{Frame from MIMIC Pick and Place exercise}
\end{figure}

\begin{table}[H]
\begin{tabular}{|l|l|}
\hline
\textbf{Feature}             & \textbf{Mean Movement} \\ \hline
Tool Camera Pitch            & 0                      \\ \hline
Tool Camera Roll             & 0                      \\ \hline
Tool Camera X                & 0                      \\ \hline
Tool Camera Y                & 0                      \\ \hline
Tool Camera Yaw              & 0                      \\ \hline
Tool Camera Z                & 0                      \\ \hline
Tool Left Jaw Opening Angle  & 0.003162               \\ \hline
Tool Left Pitch              &                        \\ \hline
Tool Left Roll               & 0.003628               \\ \hline
Tool Left X                  & 0.015099               \\ \hline
Tool Left Y                  & 0.014671               \\ \hline
Tool Left Yaw                & 0.003408               \\ \hline
Tool Left Z                  & 0.020905               \\ \hline
Tool Right Jaw Opening Angle & 0.001955               \\ \hline
Tool Right Pitch             & 0.002691               \\ \hline
Tool Right Roll              & 0.004513               \\ \hline
Tool Right X                 & 0.016174               \\ \hline
Tool Right Y                 & 0.017899               \\ \hline
Tool Right Yaw               & 0.002792               \\ \hline
Tool Right Z                 & 0.019928               \\ \hline
\end{tabular}
\caption{MIMIC kinematic features}{The kinematic positional features from the MIMIC simulator along with the absolute average change observed in subsequent timesteps computed from a single kinematic log.}
\label{tab:my-table}
\end{table}


\begin{figure}[!tbph]
  \centering
\includegraphics[width=\textwidth]{imgs/jigsaws.png}
\caption[JIGSAWS emulated surgery]{Three frames from JIGSAWS dataset; (left) suturing, (middle) knot-tying (right) needle passing.}
\end{figure}


\section{Task and Surgeon Prediction from Kinematic Data}

Using the MIMIC simulator dataset described in \ref{mimic-data}, deep learning models were trained to predict two ground truth labels easily extracted from the kinematic logs. The logs begin in the format of 30 positional recordings per second describing the location and configuration of the camera and apertures. This is converted from positional data at each timestep to the difference or movement between timesteps. While the accuracy of the models trained on these movements was good, the further step of converting movements to binary events was taken. All movements above a small threshold are coded as an event for that feature. While this results in an overall loss of information, the motivation is guided twofold; (1) the capture rate of events is sufficient that the micro movements between subsequent timesteps may be primarily operator or sensor noise and (2) encoding the data stream as binary \emph{spikes} dramatically increases the sparsity of the data, potentially greatly reducing any memory or computation footprints, and directly enabling an efficient spike-time encoding for use with neuromorphic hardware described in \ref{neuro-intro}. 

\begin{table}[H]
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Partition} & \textbf{Surgeon} & \textbf{Task} & \textbf{Task-Surgeon} & \textbf{Task-Convolution} \\ \hline
Train Accuracy     & 0.9015           & 0.9110        & 0.9141                & 0.9283                    \\ \hline
Test Accuracy      & 0.8227           & 0.8932        & 0.8810                & 0.8593                    \\ \hline
\end{tabular}

\caption[Kinematic predictive model accuracy]{Results from 4 selected trained models. In the Surgeon and Task models, data was stratified only by the label. In the Task-Surgeon model the predicted label was the surgical task but the data was partitioned by surgeon, with 1 surgeon being held out for validation. In the Task-Convolution model the LSTM layer was replaced by a 1 dimensional convolutional layer with filters equal to the number of neurons in the LSTM.}
\label{tab:mimc-res}
\end{table}

Table \ref{tab:mimc-res} shows the results of two model architectures on the two previously defined tasks. These results serve a fair baseline for two easily understood tasks on our in-house dataset with no external data. While the accuracy is not perfect, this is to be expected for a couple of reasons. First, the dataset size is still relatively small. To avoid issues with low-example labeled classes only contributing noise to the model, only the 3 tasks and 4 surgeons with the highest number of examples were used. Second, the sequences extracted from the kinematic data are short and can not capture  complex, long-range action associations. Therefore many  of these mini-action sequences should be common across both tasks  and surgeons.  Very likely with more classes we should see decreased performance, but more separable and recognizable clusters of common as well as unique action sequences. Such clusters may begin to be observed in figures \ref{fig:task-vis} and \ref{fig:surg-vis}.

\begin{figure}[!tbph]
  \centering
\includegraphics[width=\textwidth]{imgs/TaskVis.png}
\caption{Visualization of task based encoding}
\label{fig:task-vis}
\end{figure}

\begin{figure}[!tbph]
  \centering
\includegraphics[width=\textwidth]{imgs/SurgeonVis.png}
\caption{Visualization of surgeon based encoding}
\label{fig:surg-vis}
\end{figure}

These visualizations were computed by taking the activation outputs from the fully-connected layer in the network immediately preceding the output softmax layer. Each dot is a 2 second sequence of kinematic log time steps. The full sequence of processing steps are below:

\begin{itemize}
    \item Kinematic logs converted to a sequence of binary “events”
    \item Event sequences fed as input to the trained deep learning model and output by the layer preceding the output of the neural network.
    \item The 16 dimensional vector the network outputs is then decomposed to 2 dimensions with a method called TSNE which is similar to principle components analysis (PCA).
    \item These are plotted on the graph and color coded according to the ground truth label used to train the model.
\end{itemize}

We may observe in 2D the separability of the classes, as well as clusters of similar actions across 2 or more classes. This is particularly noticeable for the surgeon prediction visualization \ref{fig:surg-vis} which has a cluster almost for every combination of 2 and more surgeons. Also of note is the difference in spread of the surgeons, for example Valle and Roberto. Roberto's actions are fairly tightly distributed, while Valle's are spread farther apart even though they completed the same surgical tasks. This may indicate that Roberto's actions are more precise and consistent, or some other surgical stylistic features we may uncover.

\begin{figure}[!tbph]
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{imgs/TaskConf.png}
    \caption{Confusion matrix for task prediction}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{imgs/SurgeonConf.png}
    \caption{Surgeon prediction}
     \label{fig:confusion}
  \end{minipage}
\end{figure}

The confusion matrices in \ref{fig:confusion} show where the mistakes of the model are being made on the validation set. In particular, we can see that mistakes are most often made between Stephen generally, particularly between Stephan and Gabriella. As we train models to more precisely annotate actions, gestures, styles and skills, we may uncover why these mistakes are being made.

It is above all these learned representations of kinematic sequences that we are interested in. While we may rely on manual annotations of gestures, actions, mistakes etc. in other datasets, we may not expect a model to immediately generalize to all unseen surgical procedures and tasks. By first learning a representation of the data using supervised learning with labels that are readily available, we may increase generalizability and accuracy for downstream tasks.
